Two-loop amplitudes for ttH production: the quark-initiated Nf-part

We present numerical results for the two-loop virtual amplitude entering the NNLO corrections to Higgs boson production in association with a top quark pair at the LHC, focusing, as a proof of concept of our method, on the part of the quark-initiated channel containing loops of massless or massive quarks. Results for the UV renormalised and IR subtracted two-loop amplitude for each colour structure are given at selected phase-space points and visualised in terms of surfaces as a function of two-dimensional slices of the full phase space.

==> diagrams/1loop/Diagram8.tex <==
% Created with FeynGame
% Include with input{./diagrams/1loop/Diagram8.tex}
% Width can be set with \def\svgwidth{...} and a scaling with \def\svgscale{...}
% These options have to be set before the import statement and only apply to one included file
\begingroup%
  \makeatletter%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{595.32000732bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \parbox[c][][c]{\unitlength}{%
    \begin{picture}(1,0.41843220338983056)%
      \put(0,0){\includegraphics[width=\unitlength,viewport = 0 0 450 188]{./diagrams/1loop/Diagram8.eps}}%
      \put(0.12129237288135593,0.3294491525423729){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{${q}$}}}}}}%
      \put(0.12129237288135593,0.1138771186440678){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$\bar{{q}}$}}}}}}%
      \put(0.863559318422261,0.023834745762711863){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{${t}$}}}}}}%
      \put(0.863559318422261,0.3188559322033898){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{$\bar{{t}}$}}}}}}%
      \put(0.863559318422261,0.17002118644067796){\raisebox{-0.5\height}{\rotatebox{0.0}{\scalebox{1.0}{\makebox(0,0)[]{{${H}$}}}}}}%
    \end{picture}%
  }%
\endgroup%

